Injecting knowledge into language generation: a case study in auto-charting after-visit care instructions from medical dialogue

Factual correctness is often the limiting factor in practical applications of natural language generation in high-stakes domains such as healthcare. An essential requirement for maintaining factuality is the ability to deal with rare tokens. This paper focuses on rare tokens that appear in both the source and the reference sequences, and which, when missed during generation, decrease the factual correctness of the output text. For high-stake domains that are also knowledge-rich, we show how to use knowledge to (a) identify which rare tokens that appear in both source and reference are important and (b) uplift their conditional probability. We introduce the ``utilization rate'' that encodes knowledge and serves as a regularizer by maximizing the marginal probability of selected tokens. We present a study in a knowledge-rich domain of healthcare, where we tackle the problem of generating after-visit care instructions based on patient-doctor dialogues. We verify that, in our dataset, specific medical concepts with high utilization rates are underestimated by conventionally trained sequence-to-sequence models. We observe that correcting this with our approach to knowledge injection reduces the uncertainty of the model as well as improves factuality and coherence without negatively impacting fluency.

==> figures/qualexamples.tex <==
\begin{table*}[]
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}cll@{}}
\toprule
\multicolumn{2}{c}{\textbf{Test data}} & \multicolumn{1}{c}{\textbf{Generations}} \\ \midrule
Source &
\begin{tabular}[c]{@{}l@{}} I recommend you to take claritin daily for a few days \\ and add flonase spray to decreased the pressure in \\ upper airway and your ear \end{tabular} 
&{\begin{tabular}[c]{l} {
Baseline: Recommend claritin days add flonase spray \\ decreased pressure upper airway ear\\  
\
\\ Semantic weighted (ours): Recommend claritin and \\ flonase spray to decrease pressure} 
\end{tabular}}&  \\ 
Reference & \begin{tabular}[c]{@{}l@{}}Over the counter anti-allergic medications like Claritin \\ and Flonase spray may be helpful.\end{tabular} &  \\
\midrule
Source & 
\begin{tabular}[c]{@{}l@{}}Continue taking your Vienva every day for now , \\ and get tested for STD and pregnancy\end{tabular} 

& {\begin{tabular}[c]{l}
Baseline: Undergo std testing and and women health exam\\ 
DBA: Continue taking your vienva every day\\ 
Unweighted (ours): Undergo std and pregnancy test\\ 
Concept weighted (ours): Undergo std and pregnancy test\\
Semantic weighted (ours): Continue taking every day
\end{tabular}} &\\
Reference & \begin{tabular}[c]{@{}l@{}}Get tested for STD and pregnancy. You can do this \\ with your current primary care doctor\end{tabular} &  \\ \midrule

Source & \begin{tabular}[c]{@{}l@{}}In the meantime , try to eat bananas , and drink citrus \\ products to add potassium to your diet\end{tabular} &
{\begin{tabular}[c]{@{}l@{}}
Baseline: Continue the health diet\\ 
DBA: You will require repeat labs to check your potassium \\ level again\\
Unweighted (ours): Continue the health diet\\ 
Concept weighted (ours): You will require repeat labs to \\ check your potassium level again\\ 
Semantic weighted (ours): You will require repeat labs to \\ check your potassium level again\end{tabular}} \\
Reference & Eat potassium rich foods &  \\ \midrule

Source & \begin{tabular}[c]{@{}l@{}}There is an antibiotic called Doxycycline which \\ I can prescribe to cure the infection\end{tabular} & 
{\begin{tabular}[c]{@{}l@{}}Baseline: Take antibiotics as\\ 
DBA: Doxycycline\\
Unweighted (ours): Take doxycycline as needed\\ 
Concept weighted (ours): Doxycycline has been \\ prescribed for you\\
Semantic weighted (ours): Take doxycycline as \\ directed to cure\end{tabular}} \\
Reference & \begin{tabular}[c]{@{}l@{}}Doxycycline 100 mg oral tablet has been prescribed \\ for you.\end{tabular} &  \\ \bottomrule
\end{tabular}}
\caption{Qualitative examples from the testset comparing different methods. In each block,  we present a source dialog turn (source), and the reference careplan instruction for that turn (reference). In the last column, we show the generated care plan instruction for the source by the different methods. You can see how our final model (semantic weights) provides more detailed instructions including  capturing medical concepts correctly.}
\label{tbl:qual}
\end{table*}


==> sections/dialog_example_old.tex <==

\begin{table}[!ht]
	\footnotesize
	\def\arraystretch{1.4}%
	\hspace*{-0.25cm}
	\begin{tabular}{|p{\linewidth}|}
		\hline
		\multicolumn{1}{|p{\linewidth}|}{\textbf{Dialogue.}} \\
$\dots$  ~~~~[\textit{12 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{purple}{For the sore throat and any cough, you can try OTC cough medicine, but in experience it is not any more effective than home remedies.} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{blue}{I also recommend gargling with warm salt water, that will help with the throat inflammation.} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} Yes, I generally recommend giving it a week, and during that time continue to gargle with warm salt water, taking motrin and tylenol as needed for pain, 
\textcolor{green}{drinking/eating soft food so it doesnt irritate your throat} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{blue}{Please do gargle with the warm salt water as discussed, that will help the swelling more.} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{teal}{One more recommendation is to try TheraFlu cold and cough - its available over the counter - and will help with pain and congestion as well.} \\ 
$\dots$  ~~~~[\textit{7 dialogue turns are abbreviated from here}].~~~~ \\ \hline 
\textbf{Care plan instructions} \\
Medication Plan: \textcolor{purple}{Take Ibuprofen or Tylenol as needed, as directed, for pain.} \\
Medication Plan: \textcolor{teal}{Take TheraFlu Cold and Cough, available over the counter, as needed, as directed, for pain and congestion.} \\
Instruction: \textcolor{blue}{Gargle with warm salt water several times a day to help throat inflammation.} \\
Instruction: \textcolor{green}{Avoid any harsh or irritating foods that may worsen or further irritate your sore throat.} \\ \hline 
	\end{tabular}
	\vspace*{2mm}\caption{A sample of patient-provider dialogue. \textbf{MD} stands for provider. Only provider's turns that specify an instruction for the patient are preserved for brevity. The complete version of this dialogue can be found in appendix \ref{}. \TODO{Is the instruction generated by our model? If so, did the model learn OTC-> tyleonol? Maybe its the third MD comment}} 
	\label{table:cp-example}
\end{table}


==> sections/intro_old.tex <==
\section{Introduction}
%% medical domain


[MEDICAL INTRODUCTION AND S2S APPLICATIONS HERE] 

In particular, automatic care plan generation problem requires a well-performing sequence-to-sequence model. A care plan is a set of actions (\textit{instructions}) that providers ask the patients to do, e.g., list of medication with appropriate directions, medical examinations to undergo at the local hospital, or educational information for prevetive care. Care plan is written based on based on the concerns the patient expresses during the one-on-one conversation with physisian. The completed care plan is then stored in the electronic health record (EHR), so patient always has access to the instructions assigned by the doctor. 
In general, an instruction is a concise call-to-action phrase that summarizes some part of a discussion. For every conversation there may be one or more instructions. See table \ref{table:cpexample} for an example.

Despite the number of possible applications, sequence generation remains a challenging NLP problem. Nowadays, large pre-trained language models that tend to generate coherent text hold the state-of-the-art status for a large number of datasets. However, such models are prone to hallucinations \citep{maynez-etal-2020-faithfulness}, i.e., adding information not present in the source text, and generating degenerate outputs, e.g., premature or repetitive sequences \citep{kulikov2021characterizing, stahlberg2019nmt, holtzman2019curious, Welleck2020Neural}. 

This issue is critical for the medical data, [WHY]. Thus, sequence-to-sequence approaches, unless carefully controlled, are not being used in production for medical companies. 

While standard sequence-to-sequence approaches fail to demonstrate high precision, we believe that they can benefit from additional domain-relevant knowledge. Healthcare is a knowledge-rich area, with a lot of publicly available ontologies, lists of medical concepts. 

In this project we propose a way to tackle the issues of the sequence-to-sequence approaches for care plan generation task by incorporating the UMLS \citep{UMLS} medical concepts (medication names, findings, diseases, etc.), concept semantic types, and importance directly into the model.

We first introduce and investigate the knowldege utilization rate, and find out transformer model generates UMLS concepts significantly underutilizes the vital medical terms in its output. We empirically show the correlation between marginal probability and model's utilization rate drop.

\begin{table}[!ht]
	\footnotesize
	\def\arraystretch{1.4}%
	\hspace*{-0.25cm}
	\begin{tabular}{|p{\linewidth}|}
		\hline
		\multicolumn{1}{|p{\linewidth}|}{\textbf{Dialogue.}} \\
$\dots$  ~~~~[\textit{12 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{purple}{For the sore throat and any cough, you can try OTC cough medicine, but in experience it is not any more effective than home remedies.} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{blue}{I also recommend gargling with warm salt water, that will help with the throat inflammation.} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} Yes, I generally recommend giving it a week, and during that time continue to gargle with warm salt water, taking motrin and tylenol as needed for pain, 
\textcolor{green}{drinking/eating soft food so it doesnt irritate your throat} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{blue}{Please do gargle with the warm salt water as discussed, that will help the swelling more.} \\
$\dots$  ~~~~[\textit{5 dialogue turns are abbreviated from here}].~~~~ \\
\textbf{MD:} \textcolor{teal}{One more recommendation is to try TheraFlu cold and cough - its available over the counter - and will help with pain and congestion as well.} \\ 
$\dots$  ~~~~[\textit{7 dialogue turns are abbreviated from here}].~~~~ \\ \hline 
\textbf{Care plan instructions} \\
Medication Plan: \textcolor{purple}{Take Ibuprofen or Tylenol as needed, as directed, for pain.} \\
Medication Plan: \textcolor{teal}{Take TheraFlu Cold and Cough, available over the counter, as needed, as directed, for pain and congestion.} \\
Instruction: \textcolor{blue}{Gargle with warm salt water several times a day to help throat inflammation.} \\
Instruction: \textcolor{green}{Avoid any harsh or irritating foods that may worsen or further irritate your sore throat.} \\ \hline 
	\end{tabular}
	\vspace*{2mm}\caption{A sample of patient-provider dialogue. \textbf{MD} stands for provider. Only provider's turns that specify an instruction for the patient are preserved for brevity. The complete version of this dialogue can be found in appendix \ref{}.}
	\label{table:cp-example}
\end{table}


==> sections/old/2-background.tex <==
\section{Background}

\paragraph{Automatic care plan generation} In this paper, we tacke the problem of automatic care plan generation. 

We use a dataset $D = \{(\textbf{x}^i, \textbf{y}^i \}_{i=1}^N$, where $\textbf{x}$ (source) refers to a span of text in the dialogue that discusses the action, $\textbf{y}$ (reference) is a human-written care plan instruction corresponding to the span. 

Thus, we aim to generate a care plan instruction given a relevant dialogue turn, which is a special healthcare-tailored case of paraphrase problem. Such problems are typically solved with neural sequence-to-sequence models.

\paragraph{Sequence-to-sequence models} Neural language generation (NLG) models approximate a conditional distribution over a target vocabulary given the source sequence. Nowadays sequence-to-sequence is an umbrella term covering different model designs which are all using large-scale neural networks trained end-to-end on a finite set of pairs of texts.
In this work we consider autoregressive design of the language model.  It assumes that the probability of a sequence $\mathbf{y}$ of length $T$ is decomposed into a product of conditional probabilities given some input sequence $\mathbf{x}$:
\begin{align}
\label{eq:chainrule}
	p(\mathbf{y}|\mathbf{x}) = \prod_{i=1}^{T} p(y_i|\mathbf{y}_{<i}, \mathbf{x}),
\end{align}
where both source and reference tokens are from either shared or separated vocabulary sets.

\paragraph{Training} The neural network is used to model conditional distribution $p(y_i|\mathbf{y}_{<i}, \mathbf{x}, \theta)$ from \autoref{eq:chainrule} where $\theta$ corresponds to a set of learnable parameters of the neural network. Maximum likelihood is a de-facto standard criterion to train the model. It maximizes the log-likelihood of sentence pairs which is equivalent to minimizing the negative log-likelihood loss:
\begin{align*}
    l_\text{nll}(\theta) &= - \frac{1}{N} \sum_{n=1}^{N} \log p(\mathbf{y}^n|\mathbf{x}^n; \theta),\\
    \theta &\longrightarrow \arg\min_{\theta^\prime} l(\theta^\prime),
\end{align*}

\paragraph{Generation} After training is done the maximum-a-posteriori (MAP) decision rule is used to select the sequence which maximizes conditional probability of the hypothesis given the source text: $\hat{\mathbf{y}} = \arg \max_{\mathbf{y}} p(\mathbf{y}|\mathbf{x}; \theta)$. Solving this optimization problem exactly is intractable in most cases and approximate decoding strategies such as beam search are used in order to find the set of candidates $\mathcal{Y}_\text{beam}$ to choose from: $\hat{\mathbf{y}} = \arg \max_{\mathbf{y} \in \mathcal{Y}_\text{beam}} p(\mathbf{y}|\mathbf{x}; \theta)$.
Beam search limits search space expansion to the predefined beam width or beam size $k$.


==> sections/old/abstract-old.tex <==
Many medical applications can benefit from sequence generation models. However, autoregressive sequence-to-sequence models often misrepresent factual details of the source text and produce empty or repetitive outputs. This problem is critical for the medical domain, where factual errors can lead to severe consequences. However, healthcare is a knowledge-rich area, with handcrafted ontologies that include names of medications, exams, and findings. In this paper, we tackle the problem of factual errors in sequence generation by inducing external knowledge into the model. In particular, we stick to the UMLS \cite{UMLS} ontology as a source of medical knowledge. We quantify the model's inability to generate correct medical terms by introducing the knowledge utilization rate and show that it correlates with the marginal probability of a medical concept. We propose to explicitly maximize this marginal probability during training, and consider three ways of weighting the concepts based on their utilization rate. We study the effect of the suggested regularization on the care plan generation task for patient-provider dialogue data. A care plan is a structured to-do list that the provider shares with the patient based on their conversation, which we aim to generate automatically given the dialogue script. We observe that knowledge exploitation reduces the uncertainty of the model, and improves factuality and coherence. Our approach outperforms constrained decoding strategies, which we confirm by conducting human evaluation performed by medical experts.


%%% med applic require generation tasks. ... has these problems. .. domain is rich area, ontologies. tacklwe the generation problems. ....
%%% care plan charting, which is ...
%%% results and findings

%%% Exploit medical knowledge where available 
%%% seq2seq lacks factuality, degeneracies
%%% Correctness is critical for medical applications
%%% Knowledge-rich area, and how we induce this knowledge 
%... method 1-2 liner
%%% Care plan geenration based on the dialogue data, which is an action list of instructons that were already ...
%... results 1-2 liner
%%% 

%%Neural autoregressive sequence-to-sequence models tend to misrepresent details of the original text when generating output. This problem is critical for the medical domain, where factual errors can lead to severe consequences. In this work, we aim to tackle the problem of factuality with respect to low-frequency medical concepts, such as medications, medical examination names, findings, etc. 

%We first confirm the high discrepancy between the conditional and marginal distribution of the rare-occurring tokens. Next, we quantify this discrepancy by introducing the knowledge utilization rate, and confirm that beam search ignores the low-frequency tokens if their rate is high. We propose to incorporate the knowledge about the crucial concepts by explicitly maximizing the marginal probability under the model. We study the effect of the suggested regularization on the care plan generation task and observe two main findings. 


%First, adding more knowledge to the model helps to push up the marginal probability of infrequent tokens. This lowers the entropy of the conditional distribution on early time steps. Thus, it reduces the data-defined uncertainty of the model.
%Second, we observe both factuality and coherence improvement when the proposed regularization scheme is used. Our approach outperforms previous methods of constraining the model for the care plan generation. We confirm this observation by conducting human (medical experts) evaluation. 

==> sections/old/paraphrase_old.tex <==
By utilizing segmentation model built by MLR and medical concepts extractor, we end up with the following problem setup. We utilize a dataset $D = \{(\mathbf{x}^i, \mathbf{y}^i, C^i)\}_{i=1}^N$, where $\mathbf{x}$ (source) refers to a span of text in the dialogue that discusses the action, $\mathbf{y}$ (reference) is a human-written care plan instruction corresponding to the span, and $C^i$ is a list of medical concepts that occur in $x$. Each medical concept $c^i_j = (n^i_j, t^i_j) \in C^i$ is a pair of its name $n^i_j$ and category $t^i_j$. Not all of the concepts from $C^i$ may be present in $\mathbf{y}$. See table \ref{table:xsumex} for examples.


We approach this problem in the context of paraphrasing in which the goal is to model a conditional distribution over a target vocabulary given the source sequence. The paraphrase task aims to generate a structured sequence given an unstructured prompt. Nowadays seq2seq is an umbrella term covering different model designs which are all using large-scale neural networks trained end-to-end on a finite set of pairs of texts.
In this work we consider autoregressive design of the language model.  It assumes that the probability of a sequence $\mathbf{y}$ of length $T$ is decomposed into a product of conditional probabilities given some input sequence $\mathbf{x}$:
\begin{align}
\label{eq:chainrule}
	p(\mathbf{y}|\mathbf{x}) = \prod_{i=1}^{T} p(y_i|\mathbf{y}_{<i}, \mathbf{x}),
\end{align}
where both source and reference tokens are from either shared or separated vocabulary sets.

\paragraph{Training} The neural network is used to model conditional distribution $p(y_i|\mathbf{y}_{<i}, \mathbf{x}, \theta)$ from \cref{eq:chainrule} where $\theta$ corresponds to a set of learnable parameters of the neural network. Maximum likelihood is a de-facto standard criterion to train the model. It maximizes the log-likelihood of sentence pairs which is equivalent to minimizing the negative log-likelihood loss:
\begin{align*}
    l_\text{nll}(\theta) &= - \frac{1}{N} \sum_{n=1}^{N} \log p(\mathbf{y}^n|\mathbf{x}^n; \theta),\\
    \theta &\longrightarrow \arg\min_{\theta^\prime} l(\theta^\prime),
\end{align*}

\paragraph{Generation} After training is done the maximum-a-posteriori (MAP) decision rule is used to select the sequence which maximizes conditional probability of the hypothesis given the source text: $\hat{\mathbf{y}} = \arg \max_{\mathbf{y}} p(\mathbf{y}|\mathbf{x}; \theta)$. Solving this optimization problem exactly is intractable in most cases and approximate decoding strategies such as beam search are used in order to find the set of candidates $\mathcal{Y}_\text{beam}$ to choose from: $\hat{\mathbf{y}} = \arg \max_{\mathbf{y} \in \mathcal{Y}_\text{beam}} p(\mathbf{y}|\mathbf{x}; \theta)$.
Beam search limits search space expansion to the predefined beam width or beam size $k$.


==> sections/old/smoothing_old.tex <==
\paragraph{Why sequence-to-sequence models fail to utilize knowledge?}

In this section, we describe the issue of lacking critical concepts in the language model output. We refer to this problem as the shortage of knowledge utilization. Medical concepts are examples of low-frequency tokens as shown in figure \ref{fig:concept_freq}. We speculate that this leads to low probabilities of these crucial tokens.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/concept_frequency.pdf}
    \caption{Average term frequency of concepts comparing to the dataset average.}
    \label{fig:concept_freq}
\end{figure}


Instead of analyzing the probabilities themselves, we examine the average rank of concepts. By rank $r_t(y, \mathbf{y})$ of token $y$ at timestep $t$ for a sequence $\mathbf{y}$ we mean order number in a sorted (w.r.t. its probability $p(y|\mathbf{y}_{<t}, \mathbf{x})$) list of tokens.

We define the oversmoothing in close relation to the size of the beam used for approximate decoding. 

\begin{definition}[oversmoothing of token $y$ given the beam size $b$]
The probability of token $y$ is underdmoothed if 
\begin{align}
    \frac{1}{\sum_{i=1}^N |\mathbf{y}^i|}\sum_{i=1}^N\sum_{t=1}^{|\mathbf{y}^i|} r_t(y, \mathbf{y^i}) \mathcal{I}[\mathbf{y}^i_t = y] > b
\end{align}
\end{definition}

Thus, the undersmoothed tokens are unlikely to be generated since they fall out of the beam window. We speculate that this happens with dataset-level infrequent tokens. We assume that due to the denominator of the softmax function, the probabilities of the infrequent tokens are largely pushed down on every time step by the criterion. 

In our case, a major part of infrequent tokens consists of terms and medical concepts. Hence, if a language model tends to de-prioritize them, we end up lacking the medical precision of generated outputs.

\subsection{Maximizing the marginal probability proxy}

As oversmoothing is defined as an indicator and depends on the beam size used, we cannot optimize it directly. We instead propose to optimize a marginal probability $p(y|\mathbf{x})$ assuming that any relevant token occurring in the sequence $x$ should have a larger marginal probability than any token not present in the reference. 

Although the model cannot directly compute a marginal probability, we can approximate it through the Monte-Carlo estimation:
\begin{align}
    p(y|\mathbf{x}) = \sum_{\mathbf{y}_{<t}} p(y|\mathbf{y}_{<y}) p(\mathbf{y}_{<t}) \approx \sum_{t=1}^{|\mathbf{y}|} p(y|\mathbf{y}_{<t})p(\mathbf{y}_{<t}) \approx \frac{1}{|\mathbf{y}|}\sum_{t=1}^{|\mathbf{y}|} p(y|\mathbf{y}_{<t})
\end{align}

Thus, by maximizing the marginal probability $p(y|\mathbf{x})$ we force the rank of the token $y$ for all timesteps. 

\subsection{Oversmoothing loss for medical concepts}

We must ensure that we apply the marginal probability proxy only for a limited set of crucial tokens. For care plan generation we care about precisely generating medical concepts that we have already pre-computed in the data. For simplicity, throughout the section, we assume that every concept consists of one token only. In practice, if the concept is compound, we apply the same techniques for every token of the concept, and average the results. Thus, we define an unweighted oversmoothing loss for medical concepts:

\begin{definition}[Unweighted oversmoothing loss for medical concepts for sequence]
The unweigthed oversmoothing loss for medical concepts $C=\{c_1, c_2, \dots, c_m\}$ in a sequence $\mathbf{y}$ is defined as
\begin{align}
    l_{\text{u}}(\mathbf{y}) =  \sum_{i=1}^{m} \log \left(\frac{1}{|\mathbf{y}|} \sum_{t=1}^{|\mathbf{y}|} p(c_i|\mathbf{y}_{<t})\right)
\end{align}
\end{definition}

We also consider a weighted oversmoothing loss, in which we assign different weights to the concepts based on their categories. We empirically calculate $w_c = p(t_c|c \in \mathbf{x} \text{ and } c \in \mathbf{y})$ where $c$ is a medical concept, and $t_c$ is its category. The outlined weights show the probability that provider included the mentioned concept in the care plan. The probability is aggregated by categories. 

We then construct a weighted oversmoothing loss as follows:

\begin{definition}[Unweighted oversmoothing loss for medical concepts for sequence]
The unweigthed oversmoothing loss for medical concepts $C=\{c_1, c_2, \dots, c_m\}$ in a sequence $\mathbf{y}$ is defined as
\begin{align}
    l_{\text{w}}(\mathbf{y}) = - \sum_{i=1}^{m}  w_{c_i} \log \left(\frac{1}{|\mathbf{y}|} \sum_{t=1}^{|\mathbf{y}|} p(c_i|\mathbf{y}_{<t})\right)
\end{align}
\end{definition}

We use oversmoothing loss as a regularizization term and augment the objective function. We use $\alpha > 0$ to balance the strength of the regularization: 
\begin{align}
    l(\mathbf{y}) = (1 - \alpha) \cdot l_{\text{nll}}(\mathbf{y}) + \alpha \cdot l_{\text{u/w}}(\mathbf{y})
\end{align}
where $l_{\text{nll}} = -\sum_{t=1}^{|\mathbf{y}|}\log p(y_t|\mathbf{y}_{<t})$


==> sections/old/utilization_old.tex <==
In this section, we describe the issue of lacking critical concepts in the language model output. We refer to this problem as the shortage of knowledge utilization. Medical concepts are examples of low-frequency tokens as shown in figure \ref{fig:concept_freq}. We speculate that this leads to low probabilities of these crucial tokens.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/concept_frequency.pdf}
    \caption{Average term frequency of concepts comparing to the dataset average.}
    \label{fig:concept_freq}
\end{figure}


Instead of analyzing the probabilities themselves, we examine the average rank of concepts. By rank $r_t(y, \mathbf{y})$ of token $y$ at timestep $t$ for a sequence $\mathbf{y}$ we mean order number in a sorted (w.r.t. its probability $p(y|\mathbf{y}_{<t}, \mathbf{x})$) list of tokens.

We define the oversmoothing in close relation to the size of the beam used for approximate decoding. 

\begin{definition}[oversmoothing of token $y$ given the beam size $b$]
The probability of token $y$ is underdmoothed if 
\begin{align}
    \frac{1}{\sum_{i=1}^N |\mathbf{y}^i|}\sum_{i=1}^N\sum_{t=1}^{|\mathbf{y}^i|} r_t(y, \mathbf{y^i}) \mathcal{I}[\mathbf{y}^i_t = y] > b
\end{align}
\end{definition}

Thus, the undersmoothed tokens are unlikely to be generated since they fall out of the beam window. We speculate that this happens with dataset-level infrequent tokens. We assume that due to the denominator of the softmax function, the probabilities of the infrequent tokens are largely pushed down on every time step by the criterion. 

In our case, a major part of infrequent tokens consists of terms and medical concepts. Hence, if a language model tends to de-prioritize them, we end up lacking the medical precision of generated outputs.

\subsection{Minimizing the marginal probability proxy}

As oversmoothing is defined as an indicator and depends on the beam size used, we cannot optimize it directly. We instead propose to optimize a marginal probability $p(y|\mathbf{x})$ assuming that any relevant token occurring in the sequence $x$ should have a larger marginal probability than any token not present in the reference. 

Although the model cannot directly compute a marginal probability, we can approximate it through the Monte-Carlo estimation:
\begin{align}
    p(y|\mathbf{x}) = \sum_{\mathbf{y}_{<t}} p(y|\mathbf{y}_{<y}) p(\mathbf{y}_{<t}) \approx \sum_{t=1}^{|\mathbf{y}|} p(y|\mathbf{y}_{<t})p(\mathbf{y}_{<t}) \approx \frac{1}{|\mathbf{y}|}\sum_{t=1}^{|\mathbf{y}|} p(y|\mathbf{y}_{<t})
\end{align}

Thus, by maximizing the marginal probability $p(y|\mathbf{x})$ we force the rank of the token $y$ for all timesteps. 

\subsection{Oversmoothing loss for medical concepts}

We must ensure that we apply the marginal probability proxy only for a limited set of crucial tokens. For care plan generation we care about precisely generating medical concepts that we have already pre-computed in the data. For simplicity, throughout the section, we assume that every concept consists of one token only. In practice, if the concept is compound, we apply the same techniques for every token of the concept, and average the results. Thus, we define an unweighted oversmoothing loss for medical concepts:

\begin{definition}[Unweighted oversmoothing loss for medical concepts for sequence]
The unweigthed oversmoothing loss for medical concepts $C=\{c_1, c_2, \dots, c_m\}$ in a sequence $\mathbf{y}$ is defined as
\begin{align}
    l_{\text{u}}(\mathbf{y}) =  \sum_{i=1}^{m} \log \left(\frac{1}{|\mathbf{y}|} \sum_{t=1}^{|\mathbf{y}|} p(c_i|\mathbf{y}_{<t})\right)
\end{align}
\end{definition}

We also consider a weighted oversmoothing loss, in which we assign different weights to the concepts based on their categories. We empirically calculate $w_c = p(t_c|c \in \mathbf{x} \text{ and } c \in \mathbf{y})$ where $c$ is a medical concept, and $t_c$ is its category. The outlined weights show the probability that provider included the mentioned concept in the care plan. The probability is aggregated by categories. 

We then construct a weighted oversmoothing loss as follows:

\begin{definition}[Unweighted oversmoothing loss for medical concepts for sequence]
The unweigthed oversmoothing loss for medical concepts $C=\{c_1, c_2, \dots, c_m\}$ in a sequence $\mathbf{y}$ is defined as
\begin{align}
    l_{\text{w}}(\mathbf{y}) = - \sum_{i=1}^{m}  w_{c_i} \log \left(\frac{1}{|\mathbf{y}|} \sum_{t=1}^{|\mathbf{y}|} p(c_i|\mathbf{y}_{<t})\right)
\end{align}
\end{definition}

We use oversmoothing loss as a regularizization term and augment the objective function. We use $\alpha > 0$ to balance the strength of the regularization: 
\begin{align}
    l(\mathbf{y}) = (1 - \alpha) \cdot l_{\text{nll}}(\mathbf{y}) + \alpha \cdot l_{\text{u/w}}(\mathbf{y})
\end{align}
where $l_{\text{nll}} = -\sum_{t=1}^{|\mathbf{y}|}\log p(y_t|\mathbf{y}_{<t})$


==> sections/util_old.tex <==
\section{Approach} 
\label{sec:approach}

%\TODO{Our key insight is that} 

In many sequence-to-sequence tasks, certain rare concepts have a high probability to appear in the reference sequence ($\textbf{y}$) if they also appear in the source sequence ($\textbf{x}$). We call these concepts ``high utilization concepts'' ($c \in C_{\textnormal{HU}}$) and formally define them in \autoref{eq:high_utilization_concepts}. These concepts are comprised of one or more tokens $c=[\nu_0, \nu_1, ...]$. We hypothesize that \TODO{factuality} errors in many sequence-to-sequence tasks are caused by the learned model underestimating the conditional probability of high utilization concepts $\hat{p}(y_i=\nu, |\mathbf{y}_{<i}, \mathbf{x}, \nu \in c, c \in \mathbf{x},  c \in C_{\textnormal{HU}}) < p(...)$, where $\hat{p}$ denotes the model estimated probability and $p$ is the true probability. This is especially relevant in our after-visit care instructions charting task, where specific medical concepts are rare but have a high conditional probability of appearing in the reference if they are present in the source.

\begin{definition}
[High utilization tokens]
Given a universe of concepts $\mathcal{C}$, the set of high utilization concepts $C_{\textnormal{HU}}$ is defined as
\begin{align}
C_{\textnormal{HU}}=\left\{c \in \mathcal{C}: \frac{p(c\in\mathbf{y}|c\in\mathbf{x})}{p(c\in\mathbf{y})} \gg 1\right\}
\label{eq:high_utilization_concepts}
\end{align} 

\end{definition}

This key insight leads us to define two goals for this work:

\begin{enumerate}
    \item Develop a method for identifying high utilization concepts, $C_{\textnormal{HU}}$ for dataset  $\mathcal{D}= \{(\textbf{x}^i, \textbf{y}^i)\}_{i=1}^N$.
    \item Develop a method for augmenting the training procedure of a seq2seq models to correctly estimate the conditional probability of tokens forming high utilization concepts. 
\end{enumerate}

\subsection{Identifying high utilization concepts using externally provided knowledge}
\label{sec:identify-high-util}

The major challenge in identifying high utilization concepts in real datasets is that the concepts we are interested in are present in very few examples. This means that it is hard to directly estimate $p(c\in\mathbf{y}|c\in\mathbf{x})$ and $p(c\in\mathbf{y})$ from \autoref{eq:high_utilization_concepts}. However, these rare concepts can still be very impactful to the overall performance of the model. This is because, for a given reference, $\mathbf{y}$, it is unlikely that a \textit{particular} high utilization concept will be present ($\forall c\in C_{\textnormal{HU}}, p(c\in\mathbf{y})\ll1$), but it is also unlikely that \textit{no} high utilization concept will be present ($\prod_{c \in C_{\textnormal{HU}}} p(c\not\in\mathbf{y}) \ll 1$). This is well documented in the medical domain, where medical concepts have a very long-tailed distribution \citep{open-set}, yet may appear in almost every relevant sequence.

To overcome this challenge, we propose computing what we call ``utilization rate'', $r_{\phi}$, which we define in \autoref{eq:utilization_rate}. This function relies on the concept equivalence class map $\phi: C_\textnormal{sel} \rightarrow \mathcal{E}$ where $C_\textnormal{sel} \subseteq \mathcal{C}$ and $\mathcal{E}$ is a set of equivalence classes. ($\phi$,~$C_{\textnormal{sel}}$,~$\mathcal{E}$) cannot be derived from the data or the model, but instead are provided from an external source of knowledge. If $\phi$ is an identity (id) then $r_{\textnormal{id}}(c_n)= \hat{p}(c_n\in\mathbf{y}|c_n\in\mathbf{x}), (\mathbf{x},\mathbf{y})\in \mathcal{D}$.

\begin{definition}[Utilization rate]
The utilization rate of concept $c_n$ is defined as
\begin{align}
r_{\phi}(c_n) = \frac{\sum_{c\in \mathcal{C}} \sum_{j=1}^N\mathbf{I} [c \in \mathbf{x}^j, c \in \mathbf{y}^j, \phi(c)=\phi(c_n)]}{\sum_{c\in\mathcal{C}} \sum_{j=1}^N\mathbf{I} [c \in \mathbf{x}^j, \phi(c)=\phi(c_n)]}
\label{eq:utilization_rate}
\end{align} 

\end{definition}

Note that \autoref{eq:utilization_rate} combines both externally provided knowledge ($\phi$,~$C_{\textnormal{sel}}$,~$\mathcal{E}$) and dataset derived values. This allows us to inject domain specific information though a relevant choice of $\phi$. For medical tasks, we can limit $C_{\textnormal{sel}}$ to only medical concepts and to choose $\phi$ such that it maps them to their SNOMED CT semantic types (which informs our choice of $\mathcal{E}$). In our case study this narrows down 758 unique medical concepts to their 19 semantic types. 

We verify that a seq2seq model conventionally trained on our dataset  significantly underestimates the utilization rates of every single semantic type (see \autoref{fig:utilization_rate}), with the worst case (semantic type ``Activity") being underestimated by over 10x. This suggests that all medical concepts are part of high utilization concepts ($C_{\textnormal{HU}}=C_{\textnormal{sel}}$). It also means that many kinds of medical concepts that are present in the source sequence do not get generated in the output sequence, which drastically hurts medical correctness.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/utilization_rate.pdf}
    \caption{Semantic type utilization rate estimated from the training data (\textcolor{blue}{blue}), and generated by the model (\textcolor{orange}{orange}). See the model specification in the \TODO{make an autoref}. \TODO{we should have also utilization rates after regularization}}
    \label{fig:utilization_rate}
\end{figure}


\subsection{Utilization-rate-aware seq2seq training}
\label{sec:regularizer}

Our analysis in \autoref{sec:identify-high-util} shows that conventionally trained seq2seq models underestimate the utilization rate ($r_{\phi}$) for many rare concepts. While we cannot optimize the utilization rate directly, we can optimize the approximate \textbf{marginal probability} $p(y|\mathbf{x})$ of a token $y$ given a source sequence $\mathbf{x}$, as seen in \autoref{eq:marginal_prob}.

\begin{align}
    p(y|\mathbf{x}) = \sum_{\mathbf{y}_{<t}} p(y|\mathbf{y}_{<y}) p(\mathbf{y}_{<t}) \approx \sum_{t=1}^{\|\mathbf{y}\|} p(y|\mathbf{y}_{<t})p(\mathbf{y}_{<t}) \approx \frac{1}{\|\mathbf{y}\|}\sum_{t=1}^{\|\mathbf{y}\|} p(y|\mathbf{y}_{<t})
 \label{eq:marginal_prob}   
\end{align}

Given the source sequence $\mathbf{x}$, the tokens for which we aim to optimize the marginal probability are $\{\nu \in c, c \in \mathbf{x}  \cap C_{\textnormal{HU}}\}$. We define the unweighted utilization loss.
 
\begin{definition}[Unweighted utilization loss]
\begin{align}
    l_u(\mathbf{x}) = - \frac{1}{\|\{\nu \in c, c \in \mathbf{x}  \cap C_{\textnormal{HU}}\}\|}\sum_{\nu \in c, c \in (\mathbf{x}  \cap C_{\textnormal{HU}})}  \log p(\nu|\mathbf{x})
\label{eq:unweighted-utilization}
\end{align}

\end{definition}

However, not all concepts in $C_{\textnormal{HU}}$ are equally likely to appear in the reference given their appearance in the source. To better reflect we also propose a weighted utilization loss where the weight for each token is determined by its utilization rate. 


\begin{definition}[Weighted utilization loss]

\begin{align}
     l_{w}(\mathbf{x}) = - \frac{\sum_{\nu \in c, c \in (\mathbf{x}  \cap C_{\textnormal{HU}})}  r_{\phi}(c) \log p(\nu|\mathbf{x})}{\sum_{\nu \in c,c \in (\mathbf{x}  \cap C_{\textnormal{HU}})}  r_{\phi}(c)}
\label{eq:weighted-utilization}
\end{align}

\end{definition}

Note that \autoref{eq:weighted-utilization} directly injects externally provided knowledge through its dependence on $\phi$.

We use utilization loss as a regularization term and augment the objective function. We use $\alpha > 0$ to balance the strength of the regularization: 
\begin{align}
    l(\mathbf{x}, \mathbf{y}) = l_{\text{nll}}(\mathbf{y}) + \alpha \cdot l_{u\textnormal{ or } w}(\mathbf{x})
\end{align}
where $l_{\text{nll}} = -\sum_{t=1}^{|\mathbf{y}|}\log p(y_t|\mathbf{y}_{<t}, \mathbf{x})$ and $l_{u\textnormal{ or } w}$ is either $l_{u}$ from \autoref{eq:unweighted-utilization} or $l_{w}$ from \autoref{eq:weighted-utilization}.



% \subsection{\TODO{OLD TEXT BELOW, WILL BE INTEGRATED INTO THE SUBSECTIONS ABOVE}}




% % \paragraph{Medical knowledge} UMLS \citep{UMLS} ontology comprises of medical concepts, such as medication names, findings, and medical examinations. For each concept UMLS stores semantic type. For this problem, we identify a list medical concepts $C = \{c^i\}_{i=1}^M$ that occur in $D$. Each concept $c_i = (c^i_n, c^i_s)$ is a pair of concept name $c^i_n$ and semantic type $c^i_s$. Concept name $c_n$ is unique for every concept, while semantic type $c_s$ may refer to multiple concepts. In total, $C$ includes 758 medical concepts and 14 semantic types. We provide a full list of semantic types in the appendix.



% % \paragraph{Knowledge utilization rate} Correctness of medical text depends on how precise and complete it is in terms of medical concept utilization. We quantify this measure for the care plan generation by introducing the concept utilization rate:

% % \begin{definition}[Concept utilization rate]
% % The utilization rate of concept $c_n$ is defined as
% % \begin{align}
% % r_n(c_n) = p(c_n \in \mathbf{y} | c_n \in \mathbf{x}) = \frac{\sum_{j=1}^N\mathbf{I} [c_n \in \mathbf{x}^j, c_n \in \mathbf{y}^j]}{\sum_{j=1}^N\mathbf{I} [c_n \in \mathbf{x}^j]}
% % \end{align} 
% % \end{definition}

% % Thus, the utilization rate shows the empirical probability of the concept name to be preserved in the output if occurring in the source. Similarly, we define a semantic type utilization rate:

% % \begin{definition}[Semantic type utilization rate]
% % The utilization rate of concept $c_s$ is defined as
% % \begin{align}
% % r_s(c_n) = p(c_s \in \mathbf{y} | c_s \in \mathbf{x}) = \frac{\sum_{j=1}^N\sum_{i=1}^M\mathbf{I} [c^i_s=c_s, c^i_n \in \mathbf{x}^j, c^i_n \in \mathbf{y}^j]}{\sum_{j=1}^N\sum_{i=1}^M\mathbf{I} [c^i_s=c_s, c^i_n \in \mathbf{x}^j]}
% % \end{align} 
% % \end{definition}

% % Semantic type utilization rate reflects the percentage of preserved concepts of a specific semantic type. 


% % We do not expect all utilization rates to be close to 1.0, because some medical concepts may be omitted. However, medications should be always preserved and cannot be replaced. We examine the empirically estimated semantic type utilization rate distribution in \autoref{fig:utilization_rate}. We observe that several semantic types have extremely low utilization rates, while the ``MEDICATION" type only reaches ~0.65.

% % Next, we speculate that sequence-to-sequence models lack the precision to correctly generate medical concepts. Figure \ref{fig:utilization_rate} shows the semantic type utilization rate for a sequence-to-sequence model. The rate discrepancy between the generated output and references supports the hypothesis. Hence, autoregressive models struggle to keep enough medical knowledge and replace them with more frequent tokens. 

% % \paragraph{Why autoregressive models fail to preserve crucial tokens} We speculate that one of the reasons for NLG models struggling to keep vital tokens during generation is a low frequency of the concepts. Given the softmax denominator in the log-likelihood objective, the model heavily penalizes the infrequent tokens on every time step. Without an explicit injection of knowledge in the objective, the model cannot correctly determine the importance of a token. 

% % Hence, we propose to induce the information about vital medical concepts by maximizing the utilization rate during training.


% \subsection{Maximizing the utilization rate}

% In this section, we propose to tackle the problem of the medical concept underusage by maximizing a soft proxy to the utilization rate during training. 

% \paragraph{Marginal probability proxy} A sequence-level utilization rate is a probability of a medical concept from a source occurring in the reference. While we can estimate this probability at the corpus level, it makes it challenging to optimize it directly during training. 

% To come up with a soft proxy for the utilization rate, we estimate \textbf{marginal probability} $p(y|\mathbf{x})$ of token $y$ given a source sequence $\mathbf{x}$.

% Although the model cannot directly compute a marginal probability, we can approximate it through the Monte-Carlo estimation given the autoregressive setup:
% \begin{align}
%     p(y|\mathbf{x}) = \sum_{\mathbf{y}_{<t}} p(y|\mathbf{y}_{<y}) p(\mathbf{y}_{<t}) \approx \sum_{t=1}^{|\mathbf{y}|} p(y|\mathbf{y}_{<t})p(\mathbf{y}_{<t}) \approx \frac{1}{|\mathbf{y}|}\sum_{t=1}^{|\mathbf{y}|} p(y|\mathbf{y}_{<t})
% \end{align}

% Because some concepts may consist of several tokens, we propose to maximize the marginal probability of every token $v_i$ for a specific concept $c_n=(v_1, v_2, \dots, v_{|c_n|})$:
% \begin{align}
%     p(c_n|\mathbf{x}) = \frac{1}{|c_n|}\sum_{i=1}^{|c_n|} p(v_i|\mathbf{x})
% \end{align}

% Given that the source sequence $\mathbf{x}$ may contain several medical concepts $c^1_n, c^2_n, \dots, c^Q_n$, where one concept may occur multiple times, we aim to maximize the marginal probability of all such concepts.
% Thus, we get the following definition for the sequence-level soft proxy for the utilization rate (utilization loss).
 
% \begin{definition}[Unweighted utilization loss]
% The unweighted utilization loss for medical concepts $c^1_n, c^2_n, \dots, c^Q_n$ in a sequence $\mathbf{x}$ is defined as
% \begin{align}
%     l_u(\mathbf{x}) = - \frac{1}{Q}\sum_{i=1}^{Q}  \log p(c^i_n|\mathbf{x})
% \end{align}
% \end{definition}

% In case of utilization loss, all concepts are equally-weighted and require the model to preserve all of them in the reference. As mentioned above, this is not always the case: some concepts are more valuable than others. Therefore, we propose a weighted utilization loss with weights equal to their empirical utilization rates:

% \begin{definition}[Weighted utilization loss]
% The weighted utilization loss for medical concepts $c^1_n, c^2_n, \dots, c^Q_n$ in a sequence $\mathbf{x}$ is defined as
% \begin{align}
%     l_c(\mathbf{x}) = - \frac{1}{Q}\sum_{i=1}^{Q} r_c(c^i_n) \log p(c^i_n|\mathbf{x})
% \end{align}
% \end{definition}

% Finally, given the finite amount of data, and low frequency of every specific medical concept, we speculate that empirical probabilities used for computing utilization rates may be noisy. Hence, we propose to replace them with the semantic types utilization rates thus making the loss more robust.

% \begin{definition}[NAME??? Semantic-type-weighted utilization loss]
% The semantic-type-weighted utilization loss for medical concepts $c^1_n, c^2_n, \dots, c^Q_n$ with the corresponfing semantic types $c^1_s, c^2_s, \dots, c^Q_s$ in a sequence $\mathbf{x}$ is defined as
% \begin{align}
%     l_s(\mathbf{x}) = - \frac{1}{Q}\sum_{i=1}^{Q} r_s(c^i_s) \log p(c^i_n|\mathbf{x})
% \end{align}
% \end{definition}

% We use utilization loss as a regularization term and augment the objective function. We use $\alpha > 0$ to balance the strength of the regularization: 
% \begin{align}
%     l(\mathbf{x}, \mathbf{y}) = l_{\text{nll}}(\mathbf{y}) + \alpha \cdot l_{u/c/s}(\mathbf{x})
% \end{align}
% where $l_{\text{nll}} = -\sum_{t=1}^{|\mathbf{y}|}\log p(y_t|\mathbf{y}_{<t}, \mathbf{x})$

% We apply the regularized objective during the training of the model thus explicitly maximizing the utilization rate with respect to its weight. 

==> todo.tex <==
1. (DONE) Eq 1 and 2 - would be helpful to add a sentence or two to interpret the equation or share intuition about it. Also an illustrative example with real concepts would be helpful (lengthy part)

2 (DONE). L95-96 - please explain why the sparsity of concepts in the data makes it "hard to directly estimate" the quantity in Eq 1. If due to high variance, please state this 

3 (DONE). Explicitly define "I" symbol in Eq 2. Consider using stylized "1" instead of "I", which can be confused for identity 

4. (Done) L115 - "Our analysis in subsection 2.1 shows that conventionally trained seq2seq models underestimate the utilization rate (rϕ) for many rare concepts." - please substantiate this

5 (DONE). Eq 3 seems to have a typo in second term - p(ν|y<y) seems like it should be p(ν|y<t) 

6. (TBA to appendix) Please explain the steps taken to derive Eq 3 (to supplementary materials)

7. (DONE) 162 - please elaborate on concept identification process - e.g. what happens when two systems identify two concepts that have some overlap? These details may be helpful for those looking to build on this work (important, but also should be lengthy)

8. (DONE) L172 - Is this marginal probability computed based on dialogue, care instructions, or both? This detail would also help substantiate L174-175 "It also means that many kinds of medical concepts that are present in the source sequence do not get generated in the output sequence, which drastically hurts medical correctness."

9. (DONE) Section 5.2 - please clarify whether y in Eq 8 is the ground truth or not

10. (DONE) L270 - "This trade-off, however, has no negative impact on the quality" - please substantiate this claim in the same paragraph or point to the following section that does

11. (DONE) Cite (https://arxiv.org/abs/1904.09751v2) for the token-distribution mismatch intro

12. (DONE) Explicitly say that rare words are not OOV words => we do not compare with (cite papers from R2 and R3)
